SwiftSage: A Generative Agent with Fast and Slow Thinking for Complex Interactive Tasks

We introduce SwiftSage, a novel agent framework inspired by the dual-process theory of human cognition, designed to excel in action planning for complex interactive reasoning tasks. SwiftSage integrates the strengths of behavior cloning and prompting large language models (LLMs) to enhance task completion performance. The framework comprises two primary modules: the Swift module, representing fast and intuitive thinking, and the Sage module, emulating deliberate thought processes. The Swift module is a small encoder-decoder LM fine-tuned on the oracle agent's action trajectories, while the Sage module employs LLMs such as GPT-4 for subgoal planning and grounding. We develop a heuristic method to harmoniously integrate the two modules, resulting in a more efficient and robust problem-solving process. In 30 tasks from the ScienceWorld benchmark, SwiftSage significantly outperforms other methods such as SayCan, ReAct, and Reflexion, demonstrating its effectiveness in solving complex interactive tasks.

==> _fig_curve.tex <==


\begin{figure*}[t]
	\centering
    % \vspace{-2em}
	% \hspace{-2em}
	% \includegraphics[width=1.05\linewidth]{figures/curves.png} 
 \includegraphics[width=1\linewidth]{figures/final_curves.pdf} 
	\caption{\textbf{Visualizing trajectories of} \textcolor{blue}{\textbf{\swiftsage{}}}, \textcolor{red}{\textbf{\textsc{ReAct}}} \textbf{and} \textcolor{gray}{\textbf{\textsc{Oracle}}}. $X$: time steps ($0\rightarrow T$); $Y$: scores ($0\rightarrow 100$).
    Each figure displays the merged trajectories of testing variations by an agent in each task.
    Task IDs are shown at the bottom-right, and the ordering is based on \textit{*Len} in Tab~\ref{tab:main}.
% Each curve is a single trajectory by an agent in performing a task variation.
% A more efficient agent will achieve higher scores in a shorter time, resulting in curves positioned near the top-left corner. 
 % \todo{Captions will be enriched with explanations. It's a placeholder to estimate the layout and page limit for now.} 
 % \todo{note from raj: its really hard to see what's going on in here, I'd suggest looking at the plots from scienceworld etc?} \todo{Yuchen: what are the ``plots from scienceworld''? I'm not sure. Is it an api from sw? } 
 % raj: I just meant the style of the plots
 \vspace{0em}
	}
	\label{fig:curve}
\end{figure*}

 

==> sections/_alg.tex <==

\begin{wrapfigure}[26]{L}{0.5\textwidth}
\vspace{-1.7em}
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
	\small
	\nonl \textbf{Input:}  {{$\mathcal{M}$; $D$; $\mathcal{T}_q$ }} 
	
	\nonl \textbf{Output}: $Z = (Z_{q}, Z_{p}, Z_{n})$  \\ 
	\vspace{-0.5em}
	\hrulefill
% 	\nonl{\textbf{Remarks}: $\Gamma_{n}(X)$ samples $n$ unique data from $X$.} \\ ~\\
% 	\vspace{-0.5em}
	
% 	$\mathcal{T}_q \xleftarrow{}\Gamma_{1}(\mathcal{T})$ \comm{\scriptsize Pick a task to select query examples from.} \\
	
% 	$D_{\mathcal{T}_i} \xleftarrow{}  \{x| x \in D ,task(x) = \mathcal{T}_i$\} \comm{   \scriptsize A set that contains all the training data of the selected task } \\ 
    $D_{\mathcal{T}_q} \xleftarrow{} \{x \in D | x \text{ is an example of } \mathcal{T}_q \} $\\
	$Z_{q} \xleftarrow{}\operatorname{Sample}(D_{\mathcal{T}_q})$;~~
	$H_{q} \xleftarrow{}\operatorname{Sample}(D_{\mathcal{T}_q})$ \\
	$ R_Z \xleftarrow{} \operatorname{DenseRetrieve}(Z_q, D)$ \\
	\comm{\scriptsize Delete retrieved examples from the same task as queries.}\\
	$ R_Z \xleftarrow{} R_Z.\operatorname{discard}(D_{\mathcal{T}_q}) $
% 	\ForEach{$x \in R_{Z}$ } { 
%         \If{$task(x) = \mathcal{T}_i$}{$R_Z.delete(x)$}
%         % \EndIF
% 	}
	
	\ForEach{ {round}~~ } { 
	 $R_Z.\operatorname{shuffle()}$ \\ 
	 \comm{\scriptsize Split retrieved examples into $n$ groups} \\
	\{$G_1,...,G_n$\} $\xleftarrow{} R_Z.\operatorname{split()}$ \\
    \ForEach{$G_i \text{ in } \{G_1,...,G_n\} $ } { 
        $\mathcal{M}' \xleftarrow{}  \mathcal{M}.\operatorname{copy()}$ \\
        $\mathcal{M}'.\operatorname{fine\_tune}(G_i)$ \\
        % \comm{\scriptsize Fine-tune the upstream model using this group of retrieved examples.}\\
        $\ell \xleftarrow{} \mathcal{M}'.\operatorname{calc\_loss}(H_q)$ \\
        \ForEach{$x \in G_i$}{
            $scores[x].\operatorname{append}(\ell)$ ~~ \\
            \comm{\scriptsize Score each  in the group w/ the loss.} \\
        }
    }
	}
	
	
    \comm{\scriptsize Use mean group score as score for single examples} \\ 
	\ForEach{$x \in R_Z$}{
	    $score[x] \xleftarrow{} \operatorname{mean}(scores[x])$
	}
	\comm{\scriptsize Sort $R_Z$ by $score$ in increasing order.} \\
	
	$R_Z.\operatorname{sort(key:score, order:increasing)}$ \\
	$Z_p \xleftarrow{} $ \text{First $W$ items of $R_Z$} \\
% 	\comm{\scriptsize Smaller score means more positive effects on upstream model's performance on queries.}\\
	$Z_n \xleftarrow{} $ \text{Last $W$ items of $R_Z$} \\
	\caption{{\textbf{Distant Supervision Creation }}}\label{alg:ds_reranker}
\end{algorithm}
\end{minipage}
\end{wrapfigure}


